Layer Attack Unlearning: Fast and Accurate Machine Unlearning via Layer Level Attack and Knowledge Distillation

Recently, serious concerns have been raised about the privacy issues related to training datasets in machine learning algorithms when including personal data. Various regulations in different countries, including the GDPR grant individuals to have personal data erased, known as 'the right to be forgotten' or 'the right to erasure'. However, there has been less research on effectively and practically deleting the requested personal data from the training set while not jeopardizing the overall machine learning performance. In this work, we propose a fast and novel machine unlearning paradigm at the layer level called layer attack unlearning, which is highly accurate and fast compared to existing machine unlearning algorithms. We introduce the Partial-PGD algorithm to locate the samples to forget efficiently. In addition, we only use the last layer of the model inspired by the Forward-Forward algorithm for unlearning process. Lastly, we use Knowledge Distillation (KD) to reliably learn the decision boundaries from the teacher using soft label information to improve accuracy performance. We conducted extensive experiments with SOTA machine unlearning models and demonstrated the effectiveness of our approach for accuracy and end-to-end unlearning performance.

==> main/8_rebuttal.tex <==
\noindent We thank all the reviewers for their insightful comments and suggestions. %, and point out the areas that we can improve. 
We now address their comments and concerns.

%HY 모델의 class 또한 개인의 정보들의 집합이다. 그렇기 때문에 프라이버시 보호를 위해 class 단위별 삭제가 필요하다. 종교, 질병, 국적, 나이 그리고 성별등과 같은 민감한 문제가 포함된 분류 모델에서 활용될 수 있을 것으로 보여진다. 이런 서비스에서 민감한 class에 대한 데이터를 모델에서 완전히 제거해야하는 문제에서 우리의 접근 방식으로 문제를 풀 수 있을 것이다. 예를 들어 사회 관계망같은 서비스에서 컨텐츠를 분류하는 모델이 있을 때 새로운 법률적 해석으로 특정 class에 대한 제거를 요청 받을 수 있다. 이때 기존에 있던 모델을 폐기하지 않고 class-wise unlearning을 수행한 다면 사회적 비용의 발생을 절감하는 효과를 줄 수 있을 것이다.
%\textbf{(R2-Q1, R4-Q1) This paper focuses on class-wise unlearning  for privacy protection, making the connection to individual information unclear. }
%\textbf{(R2-Q1, R4-Q1) Cases of class-wise unlearning. }
%\hy{리뷰어가 납득가능한 내용으로}

\noindent \textbf{(R2-Q1, R4-Q1) Class-wise unlearning in the real world examples. }We thank R2 and R4 for the comments. In the real world, there may be requests to remove information about specific classes due to privacy and legal concerns. For example, the pre-trained ML can reveal information about a particular class, such as religion, diseases, nationality, age, gender, and more, on social networking sites, which individuals may not feel comfortable disclosing.
% We thank R2 and R4 for the comments. In real world, information about certain classes can be requested to remove, due to privacy and legal concerns. For example, the pre-trained ML can reveal information about a particular class such as religion, diseases, nationality, age, gender, etc. in social networking sites, which one may not feel comfortable in disclosing. 

Class-wise machine unlearning (MU) can provide the underlying mechanisms to forget the requested class information completely. In particular, we believe this issue is important for the socially disadvantaged group (class) or minority to protect their privacy and cope dynamically with regulations and legal/privacy concerns in AI domains.
% Class-wise machine unlearning (MU) can provide the underlying mechanisms to complete forget the requested class information. In particular, we believe this is an important issue for the socially disadvantaged group (class) or minority to protect their privacy, and to cope with dynamically involving regulations and legal/privacy concerns in AI domains.


%The classes of models also represent an aggregation of individual pieces of information. That's why class-wise unlearning is necessary for privacy protection. It appears that it can be applied in classification models involving sensitive issues such as religion, diseases, nationality, age, and gender. Our approach can provide a solution to the problem of completely removing data related to sensitive classes from the model in such services. For example, in services like social networks that classify content, there may be requests for the removal of specific classes due to new legal interpretations. In such cases, performing class-wise unlearning on the existing model rather than discarding it could reduce the social cost.

% instance-wise query가 더 높을 것이라는 말도 맞다. 그러나 프라이버시를 보존하기 위해 class 단위로 삭제해야하는 경우는 여럿 존재한다. 간단하게 MNIST의 확장으로 생각해본다면 개개인의 필기체를 인식하는 경우도 있다. 또한, 공항, 은행, 병원 등에서 회원을 식별하기 위한 face recognition 모델을 만들기도 한다. 만약 그 회원이 그곳들에서 탈퇴를 원한다면, 그 회원의 얼굴 정보를 지워야 할 것이다.
% 또한 사용자 개인화 모델들이 제공된다면 개인 정보 전체 삭제 기능으로써 필요될 것으로 보여진다. 예를 들면 개별 사용자의 개인화된 이메일을 필터링 한다고 했을 때 사용자의 요청에 따라 특정 분류에 대해서 모델 내 정보를 삭제 요청이 들어올 수 있을 것이다. 이런 시점들에서는 class-wise unlearning이 필요할 것으로 보여진다.
%\sy{As you rightly pointed out, in the real world, there may be a higher demand for instance-wise unlearning queries. However, there are numerous scenarios where, for the sake of preserving privacy, deletion needs to be performed on a class-wise basis. To illustrate with a simple example, consider an extension of MNIST, where one needs to recognize individual handwriting for personal identification. Additionally, there are situations where face recognition models are used to identify members in places like airports, banks, hospitals, and so on. If members wish to withdraw their consent for such identification, their facial information must be erased.}\hy{Furthermore, if personalized user models are provided, it seems necessary as a feature for complete deletion of personal information. For example, if a user's personalized email filtering is in place, there may be requests from users to delete model information related to specific categories, depending on the user's preferences. At such points in time, class-wise unlearning appears to be necessary.}

% 평가지표인 정확도를 기준으로 class-wise unlearning에 있어 두 정확도를 동시에 고려해야한다. retain data의 정확도는 높아야하면서 동시에 forgetting data의 정확도는 낮아야한다. 그러나 이 두 정확도를 동시에 평가하기에는 어떤 method가 더 좋은지 명확하지 않을 때가 있다. 예를 들어 두 정확도가 다 높을 때와, 둘 다 중간 정도일 때 등 어느 순간이 더 좋은 unlearning 결과인지 쉽게 판단하기 힘들다. 그리하여 우리는 두 지표를 하나의 지표로 mapping하는 함수를 만들어 평가하기 용이하게 만드는데 목적을 두었다. supplementary B에서 볼 수 있듯이 우리는 정확도를 지수 함수를 이용해 원하는 수치에 대해 더 높은 평가를 주게 만들고, 이들의 평균을 0과 1 사이로 min-max normalize를 한 것이다 in Eq. 13. max값은 2xexp(0)이 되고 min값은 2xexp(1)가 되고min-max normalize 목표 값은 USr + USf가 된다. 이로 인해 USr + USf 수치가 높을 수록 더 좋은 Unlearning 결과이라는 것을 쉽게 이해할 수 있다.

\noindent \textbf{(R2-Q2) Unlearning score. }
For evaluation, it is critical to consider both unlearning vs. retaining accuracy simultaneously. For example, we aim for high accuracy in the retain data and low accuracy in the forgetting data. However, as shown in prior research, comparing each metric may not be trivial and cannot fully characterize the overall holistic view of the performance from each unlearning method. 
% For example, \hl{it is challenging to discern the better unlearning result when both accuracies are high, low, or middle} \simon{unclear}.
% For evaluation, it is critical to consider the both unlearning vs. retaining accuracy simultaneously. For example, it is desirable to have the accuracy of retaining data high, while that of the forgetting data low. However, as shown in prior research, comparing each metric separately may not be trivial and cannot fully characterize the overall holistic view of the performance from each unlearning method. For example, \hl{it is challenging to discern the better unlearning result when both accuracy are high, low, or moderately balanced} \simon{unclear}. 

Therefore, we propose an unlearning score (US) that captures both accuracy performances into a single unified metric, making the evaluation more directly comparable, as presented in Section B in Suppl Mat. The exponential function provides higher scores w.r.t accuracy values. Then, we normalize and average them to reflect the retain and forgetting data performances better in a single value.
% Therefore, we propose an unlearning score (US) that captures the both accuracy performances into an unified single metric, making the evaluation more directly comparable, as presented in Section B in Suppl Mat. The exponential function provides higher scores w.r.t accuracy values. Then, we normalize and average them to better reflect the forgetting and retain data performance in a single value.

%Then, we average these values to a single value and min-max normalization in Eq.~\ref{eq:13}. The min value becomes ${2 \cdot \exp(0)}$, and the max value becomes ${2 \cdot \exp(1)}$, and the target value for min-max normalization is ${\text{US}_r + \text{US}_f}$. Consequently, it becomes easier to understand that a higher value signifies a better unlearning outcome.


%However, it can be more complex to determine which method is superior when considering these two accuracy concurrently.
%  T의 영향력에 대해서 말씀드리겠습니다. Table A1.에서 ResNet18의 CIFAR-10에서 T의 변화에 따른 unlearning 성능을 측정하였습니다.(In Table~\ref{tab:KD_T}, we measured the unlearning performance of ResNet18 on CIFAR-10 with varying values of T.) T의 변화에 따른 성능의 차이는 0.1-0.2% 정도였습니다. 결과와 같이 T의 영향력이 Loss function 내에서 미미하였습니다. 하지만 실험처럼 미세하지만 적절한 T의 설정으로 얻는 이득이 있기에 커맨트 주신 것 처럼 본 실험 내용을 supplementary에 추가하겠습니다. 아울러 4. Experimental Results 세션에서 우리는 T는 4로 설정하고 실험한 결과 입니다.
% Eq 7. 내 T^2은 Teacher모델로 부터 지식을 얻어오는 가중치 term입니다. 해당 term에 대한 내용을 간략하게 논문에 추가하겠습니다.

%  T의 영향력에 대해서 말씀드리겠습니다. ResNet18의 CIFAR-10에서 T의 영향력을 파악하고자 값을 1, 4, 8, 16으로 변화시켜서 실험을 수행하였습니다.(In our experiments, we set the value of T to 4, and this yielded the best performance among the choices.)(We conducted experiments on ResNet18 with CIFAR-10 to assess the impact of T by varying its values to 1, 4, 8, and 16) T의 변화에 따른 성능의 차이는 0.1-0.2% 정도였습니다. 결과와 같이 T의 영향력이 Loss function 내에서 미미하였습니다. 하지만 실험처럼 미세하지만 적절한 T의 설정으로 얻는 이득이 있기에 커맨트 주신 것 처럼 본 실험 내용을 supplementary에 추가하겠습니다. 아울러 4. Experimental Results 세션에서 우리는 T는 4로 설정하고 실험한 결과 입니다.
% Eq 7. 내 T^2은 Teacher모델로 부터 지식을 얻어오는 가중치 term입니다. 해당 term에 대한 내용을 간략하게 논문에 추가하겠습니다.
% $T^{x}$의 x를 1, 2, 4, 8로 실험을 수행하였으며 그중 best performaces는 x

\noindent \textbf{(R2-Q3/Q4) Hyper-parameter $T$. }
We thank R2 for the question. %We tried the different $T$ values, and $T$ = 4 shows the best performance.
In Eq~\ref{eq:final_loss}, $T^{2}$ represents the weight term for obtaining knowledge from the teacher model. We tried the different $T$ values, and $T$ = 4 yielded the best performance. We will incorporate a brief explanation of this term into the Ablation Study in Section 4.3.


%We conduct experiments with $x$ values of 1, 2, 3, and 4 for $T^{x}$
%, %and among them, the best performance is achieved when x is 2. 
%We will incorporate a brief explanation of this term into the Ablation Study in Section 4.3.
% \sy{We will add a brief explanation of this term to the paper. We will include this detail in the Ablation Study in Sec 4.3. we will 중복}
% We thank R2 for the question. We tried the different $T$ values and $T$ = 4 shows the best performance. We will include this detail in Ablation Study in Sec 4.3.

%We discuss the influence of T in Eq~\ref{eq:kl_loss}, Eq~\ref{eq:final_loss}. We conducted experiments on ResNet18 with CIFAR-10 to assess the impact of T by varying its values to 1, 4, 8, and 16. In our experiments, we set the value of T to 4, and this yields the best performance among the choices. The performance difference with respect to changes in T was approximately 0.1-0.2\%. As shown in the results, the influence of T was marginal within the loss function. However, as suggested in your comment, since there are benefits obtained with subtle yet appropriate T settings, we will include the details of this experiment in the supplementary section. In Eq~\ref{eq:final_loss}, $T^{2}$ represents the weight term for acquiring knowledge from the Teacher model. We will add a brief explanation of this term to the paper.

%\hy{왜 T^2인가?}

% 하이퍼 파라미터 T의 변화에 따른 unlearning 성능. ``4. Experimental Results" section 에서 사용한 하이퍼 파라미터를 bold로 표시하였다.

\iffalse
\setcounter{table}{0}
\renewcommand{\thetable}{A\arabic{table}}
\begin{table}[t]
\centering
\caption{Accuracy of T on CIFAR-10 with ResNet18.}
\label{tab:KD_T}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{c|cccc|c}
\toprule
T       & 1     & 4     & 8     & 16     &Original \\
\midrule \midrule
$D_{r}$  & 99.98 & 99.98 & 99.97 & 99.97 &99.98 \\
$D_{f}$  & 0     & 0     & 0     & 0     &100 \\
$D_{tr}$ & 93.4  & 93.53 & 93.32 & 93.24 &93.13 \\
$D_{tf}$ & 0     & 0     & 0     & 0     &96.60 \\ \bottomrule
\end{tabular}%
}
\end{table}
\fi

\iffalse
\setcounter{table}{0}
\renewcommand{\thetable}{A\arabic{table}}
\begin{table}[t]
\centering
\caption{Accuracy of $T^{x}$ on CIFAR-10 with ResNet18.}
\label{tab:KD_2T}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{c|cccc|c}
\toprule
x       & 1       & 2     & 3     & 4        &Original \\
\midrule \midrule
$D_{r}$  & 99.97  & 99.98 & 99.95 & 90.63    &99.98 \\
$D_{f}$  & 0      & 0     & 1.94  & 4.77     &100 \\
$D_{tr}$ & 93.37  & 93.53 & 92.67 & 82.09    &93.13 \\
$D_{tf}$ & 0      & 0     & 2.7   & 5.03     &96.60 \\ \bottomrule
\end{tabular}%
}
\end{table}
\fi

% 말씀하신 것과 같이 PGD는 널리 사용하고 있다. 우리의 차별점은 unlearning task에서 Partial-PGD를 활용하여 부분적으로 적대적 공격을 통해 몇 가지 이득을 취했습니다. Table7에서 보신 것과 같이 latent space에서 Partial-PGD를 적용함으로써 unlearning task에서 연산량과 정확도를 개선된 점을 확인할 수 있었습니다. 입력층에 노이즈를 추가하는 일반적 PGD에서 특정된 layer에서 노이즈를 추가하는 Partial-PGD를 unlearning task에 시도한 점이 novelty가 있다고 생각합니다. 또한 Partial-PGD은 PGD를 사용하는 다른 unlearning algorithm에 활용된다면 성능 계선을 시켜줄 수 있을 것으로 기대합니다.

%\textbf{(R3-Q1, R4-Q2) The novelty is limited given the fact that PGD already did similar things and this paper just adds noise in the latent space instead. }

\noindent \textbf{(R3-Q1, R4-Q2) The Novelty of Partial-PGD. } 
The novelty in our Partial-PGD lies in injecting noise to a specific layer for unlearning (see Fig.~\ref{fig:pgdvsppgd}.) instead of applying it to entire layers, further demonstrating that ours achieves better performance. We are the first to show that Partial-PGD provides clear benefits for computation efficiency and accuracy for the unlearning task that does not require entire back-propagation while achieving higher accuracy performance. A side-by-side comparison between PGD and Partial-PGD is provided in Table 3, where our approach achieves higher accuracy and faster unlearning time.  
% The novelty in our Partial-PGD lies in injecting noise to specific layer for unlearning (see Fig.1.), instead of applying it to entire layers, and further demonstrate that ours achieves better performance. We are the first to show that Partial-PGD provides clear benefits for computation efficiency and accuracy for unlearning task that does not require entire back-propagation, while achieving higher accuracy performance. A side-by-side comparison between PGD and Partial-PGD are provided in Table 3, where our approach achieves higher accuracy and fast unlearning time.    

%As you mentioned, PGD is widely used in practice. Our distinctive approach involves leveraging Partial-PGD in the unlearning task, which allowed us to gain some advantages through partial adversarial attacks. 

%As you can see in Table~\ref{tab:pgd_vs_partial_pgd}, applying Partial-PGD in the latent space resulted in improvements in computational efficiency and accuracy in the unlearning algorithm. We believe that the novelty lies in our attempt to apply Partial-PGD in the unlearning task by adding noise to specific layers, as opposed to the common PGD approach that adds noise to the input layer. Furthermore, we expect that Partial-PGD, if applied to other unlearning algorithms that use PGD, can lead to performance improvements.

%\textbf{(R3-Q7) Why machine unlearning cannot simply be achieved by randomly reassigning the label of the data to be forgotten to other labels, as a simpler alternative to preserve accuracy while ensuring the data is forgotten. }

% 네 말대로 forgetting data에 random label을 할당하는 것은 쉽고 직관적이다. 그러나 그러한 방법 중 하나는 baseline의 random label이다. forgetting data에 random label을 할당하여 fine-tune 하는 것은 Table1에서 보다시피 제대로 잊혀지지 않는 모습을 볼 수 있다. 또 다른 방법은 model을 fine-tune 하지 않고 원래 출력에 대해 random label을 출력하도록 보정하는 것이다. 그러나 이것은 forgetting data에 대한 정보가 모두 model에 유지되어 있기 때문에 attacker가 모델을 확보한다면 attack을 쉽게할 수 있다. (수치, 생각)

%\hy{Random Assign했을때 결과}
% 
\setcounter{figure}{0}
\renewcommand{\thefigure}{A1}
\begin{figure}[t] \centering   \includegraphics[width=0.95\columnwidth]{main/figure/logits5.pdf}
    \vspace{-0.5cm}
    \caption{Average logit values with each model on $D_{tf}$.}
    \label{fig:logits}
\vspace{-0.7cm}
\end{figure}

\noindent \textbf{(R3-Q7) Random label assignment for forgetting data. }
We thank R3 for the great question. Indeed, assigning random labels to forgetting data is a simple and intuitive approach. We have a baseline ``Random Label'' in Table 1 and compare the results. We show that our performance is better than the randomized approach, which is not the most optimized unlearning method.
% We thank R3 for the great question. Indeed, assigning random labels to forgetting data appears to be a simple and intuitive approach. We have a baseline ``Random Label'' in Table 1, and compare the result. We show that ours performance better than randomized approach which is not the most optimized unlearning method.  

% Additionally, we thank R3 for the insightful idea of rerouting and reassigning at the output layer. Indeed, we consider those cases. However, this approach is not unlearning or forgetting from the model's view point, as the model still remembers but assign to different labels. This can be a problem, when an attackers steal the model and he can fully recover the entire unlerned data, while in our approach attackers cannot recover data from our unlearned model.    
Additionally, we thank R3 for the insightful idea of re-routing at the output layer. Indeed, we consider those cases. However, this approach is not unlearning or forgetting from the model's viewpoint, as the model still remembers but re-routes to different labels. The following small experiments show the results of ``re-routing the class'' as suggested by R3.
In Fig.~\ref{fig:logits}, we compared the logit averages for 1) the Original/Re-Routing model, 2) the Retrain model, and 3) Our model with $D_{tf}$. As shown, the re-routing method yields significantly high logit values for the ``ship'' class it needs to forget at the output, while the other two methods (Retrain and Ours) distribute them more evenly with much smaller values. This means re-routing does not unlearn and still remembers the forgetting class internally. 
%In essence, the logits for re-routing method remain identical to those of the original model.
In particular, this can be a problem when an attacker steals the model and can recover the entire unlearned data, while in our approach, attackers cannot retrieve data from our unlearned model.

% 즉 Re-route에 대한 logits은 original model에서 전혀 달라지지 않았고, 이는 attacker가 attack을 위한 중요한 정보로 활용할 수 있다.
% 내가 잊고자 하는 클래스를 단순히 다른 클래스로 routing하는 것은 그 데이터의 logit은 유지가 된다는 의미이다. fig a는 the forgetting data에 대한 Original model, Retrain model, our model의 클래스별 logit 평균을 그린 것이다. fig a에서 볼 수 있듯이, Re-routing 방법은 the forgetting class에 대한 logit 값이 매우 크고, 나머지 두 방법은 비교적 고루 퍼져있다는 것을 알 수 있다.


%Another method involves adjusting the original outputs to route to random labels without fine-tuning the model. Nevertheless, this approach retains all the information about forgetting data within the model, making it vulnerable to attacks if an attacker gains access to the model.



%method in baselines. Fine-tuning with arbitrary labels for the forgetting data, as seen in Table \ref{tab:accuracy_table}, reveals that the forgetting data aren't being completely forgotten. Also, it has side effects on the retain data. Another method involves adjusting the original outputs to route to random labels without fine-tuning the model. Nevertheless, this approach retains all the information about forgetting data within the model, making it vulnerable to attacks if an attacker gains access to the model.

%맞다 훨씬 쉽고 직관적이다. 그러나 baseline에서 Random label이 당신이 말한 내용이며, 제대로 잊혀지지 않았다. 
%출력 쪽에서의 re-routing

% 해당 질문에 대해서 2가지를 생각해볼 수 있고 그것을 서술 함

%\textbf{(R4-Q3) Retrain vs. Unlearning: Time Performance on with relative small, medium size model. }
%\textbf{(R4-Q3) Retrain vs. Unlearn: Timing with Small to Medium Models. }

\noindent  \textbf{(R4-Q3) Time Perf. with small to medium Models. }
We conducted experiments using models of various sizes with a differing number of parameters: ViT (2.18M to 9M), VGG16 (14.72M), ResNet18 (11.17M), and ResNet50 (23.52M). As shown in Table 2, the retraining process takes an average of 3,188 seconds, while ours takes an average of 9.57 seconds. Additionally, in the experiments with a smaller model containing 0.4M, it takes 925 seconds for retraining from scratch, excluding $D_{f}$, while our method takes 5.05 seconds to achieve the same performance. We hope that this will address R4's concern. 
% We conducted experiments using models of various sizes with the differing number of parameters: VIT (2.18M to 9M), VGG16 (14.72M), ResNet18 (11.17M), and ResNet50 (23.52M). As shown in Table 2, the retraining process takes an average of 3,188 seconds, while unlearning takes an average of 6.35 seconds. Additionally, in the experiments with a smaller model containing 0.4M, it takes 925 sec for retraining, since it involves retraining from scratch excluding $D_{f}$, while unlearning takes 5.05 seconds. We hope that this would address R4's concern. 
%Furthermore, in Table 5, we show that unlearning was performed using only a subset of $D_{f}$, resulting in improved efficiency.

%각 모델의 파라미터의 수는 VIT는  218~900M, VGG16은 1,472M, ResNet18은 1,117M 그리고 ResNet50은 2352M이며 이와 같이 다양한 size의 model에서 실험을 수행하였다.
% Table 2에서와 같이 Retrain의 경우 평균 3,188 초가 소요됐으며 unlearning의 경우에는 평균 6.35초가 소요되었다. 추가로 40M 파라미너를 갖고 있는 작은 모델에서 실험한 결과 Retrain의 경우 처음부터 $D_{f}$를 제외하고 다시 학습하기 때문에 925초가 소요됐으며 unlearning의 경우 5초가 소요됐다. 아울러 Table 5. 에서 일부 D_f만을 사용해서 unlearning이 수행되었고 빨라진 것을 확인 할 수 있다. 

% VIT : 218M ~ 900M
% VGG16 : 1472M
% Resnet18 : 1117M
% Resnet50 : 2352M
% 더 작은 모델에서 작업?
% cifar10 & resnet18 : 11,173,962개, 53.89MB
% cifar10 & resnet50 : 23,520,842개, 155.86MB
% cifar10 & vgg16 : 14,728,266개, 62.76MB
% cifar10 & vit : 2,189,066개 23.38MB
% fashion & resnet18 : 11,172,810개, 53.87MB
% fashion & resnet50 : 23,519,690개, 155.85MB
% fashion & vgg16 : 14,727,114개, 62.75MB
% fashion & vit : 2,180,874개, 23.32MB
% vggface2 & resnet18 : 11,173,962개, 594.45MB
% vggface2 & resnet50 : 23,520,842개, 3330.42MB
% vggface2 & vgg16 : 14,728,266개, 378.51MB
% vggface2 & vit : 9,072,138개 135.65MB

% vit base (원 논문) 약 86,600,000개 흠...
% 데이터 셋에 의존도가 큰듯 합니다... patch사이즈와 개수

\noindent \textbf{(R4-Q4) An explanation of ``the model" in Sec 4. }
We thank R4 for the comment. The model refers to the models we considered VGG16, ResNet18, ResNet50, and ViT. We will clarify and make it more explicit. 

%In Section \ref{sec:experiments}, ``the model" in the middle to explain the Original and Retrain models refers to any models like VGG16, ResNet18, ResNet50, and ViT. We will also address any ambiguities in the paper.

% "The model"에 대한 설명
% 모호한 표현을 잘 지적해주었다. original과 retrain 모델을 설명하기 위해 사용된 'the model'은 임의의 DNN 모델을 의미한다. 우리의 실험에서는 vgg16, resnets, vit라고 할 수 있다.


%\textbf{(R4-Q5) In the results, why does some ``retrain" show lower $D_{r}$ compared with ``Ours"?. }
%\textbf{(R4-Q5) Some retrain show lower $D_{r}$ compared with ``Ours". }

% 당신의 날카로운 지적 고맙다. retrain시 결과의 미세한 결과의 차이는 몇 가지 요소가 있습니다. 난수성과 부동소수점의 정밀도 때문에 정확도에서  1\%  차이가 보여지는 것 같습니다. 난수성의 예시로는 가중치 초기화 및 확률적 경사하강법에서의 Mini-batch 선택에 따라 결과가 달라지는 것으로 보여집니다. 실험에서 서로 독립된 환경에서 모델을 학습시켜 난수성으로 미세한 정확도 차이가 발생된 것으로 보여집니다. 또한 이런 난수성과 함께 미세한 부동 소수점의 정밀도 문제가 작은 차이를 보인 것 같습니다. 아울러서, 표에서 볼 수 있다시피 original 모델이 Retrain 모델보다 대부분 성능이 조금 더 높다. 이는 retrain보다 학습 데이터 수가 더 많아 generalization 성능이 살짝 더 높다는 것으로 해석할 수 있다. 우리의 방법은 그 original method를 기반으로 fine-tune하는 것이기 때문에 그 generalization 성능이 남아있을 수 있다.
%\hy{Random 성에 대한 증명으로 ResNet18로 retrain 모델을 3개를 만들어서 평가}

\noindent \textbf{(R4-Q5) Some cases show lower $D_{r}$ Performance. }
We appreciate R4 for the insightful question. We repeated each experiment 5 times and average them. We tried our best to mitigate the variability in our experiments, such as running them in the same environment, etc. However, due to the stochastic nature of the stochastic gradient descent (SGD) algorithm, the retrain model may perform less. For a more detailed analysis, the original model generally outperforms the retrain model because it is trained with more training data $D_{f}$, and our model, as a fine-tuned version of the original model, retains better generalization ability.
% We appreciate R4 for the insightful question. We repeat each experiment for 5 times and average them. And, we further tried our best to mitigate the variability in our experiments such as running them in the same environment, etc. However, due to the stochastic nature of the stochastic gradient descent (SGD) algorithm and noise generation in Partial-PGD, ours possibly achieves a lower performance. In fact, the original model generally outperforms the Retrain model. And, our model is fine-tuned version of the original model, having better generalization ability. Therefore, this is also the possible reason for the lower performance. We plan to further analyze this in the future.  

%it possibly performed better due to  

%It appears that there is a 1\% difference in accuracy due to randomness and floating-point precision. Examples of randomness include differences in results based on weight initialization and the selection of mini-batches in stochastic gradient descent. In the experiments, it appears that training the models in independent environments resulted in minor accuracy differences due to randomness. Additionally, along with this randomness, slight floating-point precision issues contributed to the observed small differences. Moreover, as shown in Table \ref{tab:accuracy_table}, that the original model generally outperforms the Retrain model by a small margin. This could be attributed to the original model having more training data than the Retrain model, resulting in slightly better generalization. Since our approach is fine-tuning the original model, it retains some of that generalization performance.


%\noindent \textbf{(R4-Q5) Some retrain show lower $D_{r}$. }We appreciate R4's keen insights. It appears that there is a 1\% difference in accuracy due to randomness and floating-point precision. Examples of randomness include differences in results based on weight initialization and the selection of mini-batches in stochastic gradient descent. In the experiments, it appears that training the models in independent environments resulted in minor accuracy differences due to randomness. Additionally, along with this randomness, slight floating-point precision issues contributed to the observed small differences. Moreover, as shown in Table \ref{tab:accuracy_table}, that the original model generally outperforms the Retrain model by a small margin. This could be attributed to the original model having more training data than the Retrain model, resulting in slightly better generalization. Since our approach is fine-tuning the original model, it retains some of that generalization performance.


% retrain시 성능이 떨어지거나 다르게 나오는 case에 대한 paper가 있는지 찾아봄
% 당신의 날카로운 지적 고맙다. DNN 계열이 black-box 학습이기 때문에 1% 내외의 정확도 차이는 존재할 수 있다. 더 자세한 분석을 해보자면, 표에서 볼 수 있다시피 original 모델이 Retrain 모델보다 대부분 성능이 조금 더 높다. 이는 retrain보다 학습 데이터 수가 더 많아 generalization 성능이 살짝 더 높다는 것으로 해석할 수 있다. 우리의 방법은 그 original method를 기반으로 fine-tune하는 것이기 때문에 그 generalization 성능이 남아있을 수 있다.
%\sy{We appreciate your keen insights. Deep Neural Networks (DNNs) are often considered black-box models, which means there may be a slight difference in accuracy, typically within 1\%. A more detailed analysis reveals, as shown in Table \ref{tab:accuracy_table}, that the Original model generally outperforms the Retrain model by a small margin. This could be attributed to the Original model having more training data than the Retrain model, resulting in slightly better generalization. Since our approach is fine-tuning the Original model, it retains some of that generalization performance.}


\noindent \textbf{Minor typos. } 
We sincerely thank all the reviewers for carefully reading our manuscript and providing suggestions and questions for minor typos and errors. We will fix all of those and incorporate them in the final version.
% Sincerely, we thank all the reviewers for carefully reading our manuscript, and provide the suggestions and questions for minor typos and errors. We will fix all those and incorporate them in the final version.
%\\

\noindent \textbf{Last but not least. } We appreciate Rs for finding our work interesting and important. Also, we thank Rs for their constructive comments and suggestions to help improve our paper. We will incorporate them all in the final version.

==> main/table/multi_label_forget.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Multi-label unlearning시 정확도
\begin{table}[htp!]
\centering
\caption{Accuracy performance in the case of multi-label unlearning on the CIFAR-10 in ResNet18}
\label{tab:multi-label-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc|cccccccccc|c} \toprule
\multicolumn{2}{c|}{Class}             & 0    & 1    & 2    & 3    & 4    & 5    & 6    & 7    & 8    & 9    & Time  \\ \midrule \midrule
\multicolumn{2}{c|}{Original}          & 94   & 95.8 & 89.8 & 86.7 & 94.2 & 88.3 & 95.9 & 96.2 & 96.6 & 96.3 & -     \\ \midrule
\multicolumn{1}{c|}{}&(2,4) & 92.6 & 97.6 & 0    & 91.7 & 0    & 85   & 96.3 & 96.8 & 97.1 & 95.5 & 8.83  \\
\multicolumn{1}{c|}{Forget}&(4,6)  & 95.5 & 95.9 & 92.8 & 87.1 & 0    & 87.6 & 0    & 97.6 & 96.4 & 96.6 & 8.9   \\
\multicolumn{1}{c|}{Label}&(6,8)  & 95.5 & 96.4 & 91   & 88.3 & 94.1 & 89.4 & 0    & 95.8 & 0    & 97.1 & 9.14  \\
\multicolumn{1}{c|}{}&(7,9)   & 91.8 & 98.6 & 94.3 & 83.1 & 90   & 91.1 & 95.6 & 0    & 95.5 & 0    & 43.55 \\ \bottomrule
\end{tabular}%
}
\end{table}
